Node Embeddings and Exact Low-Rank Representations of Complex Networks

Low-dimensional embeddings, from classical spectral embeddings to modern neural-net-inspired methods, are a cornerstone in the modeling and analysis of complex networks. Recent work by Seshadhri et al. (PNAS 2020) suggests that such embeddings cannot capture local structure arising in complex networks. In particular, they show that any network generated from a natural low-dimensional model cannot be both sparse and have high triangle density (high clustering coefficient), two hallmark properties of many real-world networks. In this work we show that the results of Seshadhri et al. are intimately connected to the model they use rather than the low-dimensional structure of complex networks. Specifically, we prove that a minor relaxation of their model can generate sparse graphs with high triangle density. Surprisingly, we show that this same model leads to exact low-dimensional factorizations of many real-world networks. We give a simple algorithm based on logistic principal component analysis (LPCA) that succeeds in finding such exact embeddings. Finally, we perform a large number of experiments that verify the ability of very low-dimensional embeddings to capture local structure in real-world networks.

==> arxivSrc/broadimpact.tex <==
This paper contributes towards a better understanding of low-rank factorization, node embedding methods, and shows that a simple algorithm based on logistic PCA can output remarkably accurate low-rank factorizations.  Our work may benefit researchers and also practitioners who (i) use node embeddings for downstream machine learning and data analysis tasks, (ii) develop novel node embedding methods, and/or (iii) study the interplay between privacy and node embeddings. Our work illustrates that node embeddings can capture significant specific information about edges in a graph, highlighting potential privacy risks of e.g., releasing such embeddings for users in a social network.

We do not foresee direct negative outcomes of our work, although acknowledge that improved methods for network analysis (including those based on embeddings) have social consequences. For example, improved graph-based recommendations can contribute to issues of filter bubbles,  polarization, and the spread of false information \cite{pariser2011filter,lee2014social,musco2018minimizing}. They may also be associated with negative well-being impacts due to increased social media use \cite{verduyn2015passive,shakya2017association,verduyn2017social}
